Time-series and Phasecurve Photometry of Episodically-Active Asteroid (6478) Gault in a Quiescent State Using APO, GROWTH, P200 and ZTF

We observed Episodically Active Asteroid (6478) Gault in 2020 with multiple telescopes in Asia and North America and have found that it is no longer active after its recent outbursts at the end of 2018 and start of 2019. The inactivity during this apparation allowed us to measure the absolute magnitude of Gault of H_r = 14.63 +/- 0.02, G_r = 0.21 +/- 0.02 from our secular phasecurve observations. In addition, we were able to constrain Gault's rotation period using time-series photometric lightcurves taken over 17 hours on multiple days in 2020 August, September and October. The photometric lightcurves have a repeating $\lesssim$0.05 magnitude feature suggesting that (6478) Gault has a rotation period of ~2.5 hours and may have a semi-spherical or top-like shape, much like Near-Earth Asteroids Ryugu and Bennu. The rotation period of ~2.5 hours is near to the expected critical rotation period for an asteroid with the physical properties of (6478) Gault suggesting that its activity observed over multiple epochs is due to surface mass shedding from its fast rotation spun up by the Yarkovsky-O'Keefe-Radzievskii-Paddack effect.

==> bib.tex <==
@article{Hanus2017b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...601A.114H},
	archiveprefix = {arXiv},
	author = {{Hanu\v{s}}, J. and {Viikinkoski}, M. and {Marchis}, F. and {\v{D}urech}, J. and {Kaasalainen}, M. and {Delbo'}, M. and {Herald}, D. and {Frappa}, E. and {Hayamizu}, T. and {Kerr}, S. and {Preston}, S. and {Timerson}, B. and {Dunham}, D. and {Talbot}, J.},
	date-added = {2017-07-11 09:33:42 +0000},
	date-modified = {2018-05-25 11:09:56 +0000},
	doi = {10.1051/0004-6361/201629956},
	eid = {A114},
	eprint = {1702.01996},
	journal = {\aap},
	keywords = {minor planets, asteroids: general, techniques: photometric, methods: numerical, methods: observational},
	month = may,
	pages = {A114},
	primaryclass = {astro-ph.EP},
	title = {{Volumes and bulk densities of forty asteroids from ADAM shape modeling}},
	volume = 601,
	year = 2017,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201629956}}

@ARTICLE{Purdum_2020,
       author = {{Purdum}, Josiah and {Lin}, Zhong-Yi and {Bolin}, Bryce T. and
         {Quimby}, Robert and {Lisse}, Carey M. and {Bhalerao}, Varun and
         {Bodewits}, Dennis and {Chang}, Chan-Kao and {Deshmukh}, Kunal P. and
         {Hsu}, Chen-Yen and {Ip}, Wing-Huen and {Jones}, R. Lynne and
         {Mahabal}, Ashish and {Ngeow}, Chow-Choong},
        title = "{Recent Non-active Appearance of Episodically Active Asteroid (6478) Gault}",
      journal = {The Astronomer's Telegram},
     keywords = {Asteroid, Comet},
         year = 2020,
        month = jul,
       volume = {13885},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ATel13885....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bolin2020HST,
       author = {{Bolin}, Bryce T. and {Lisse}, Carey M.},
        title = "{Constraints on the spin-pole orientation, jet morphology, and rotation of interstellar comet 2I/Borisov with deep HST imaging}",
      journal = {\mnras},
     keywords = {comets: general, local interstellar matter, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = jul,
       volume = {497},
       number = {4},
        pages = {4031-4041},
          doi = {10.1093/mnras/staa2192},
archivePrefix = {arXiv},
       eprint = {1912.07386},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.497.4031B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Jewitt_2015,
   title={The Active Asteroids},
   ISBN={9780816532131},
   url={http://dx.doi.org/10.2458/azu_uapress_9780816532131-ch012},
   DOI={10.2458/azu_uapress_9780816532131-ch012},
   journal={Asteroids IV},
   publisher={University of Arizona Press},
   author={Jewitt, D. and Hsieh, H. and Agarwal, J.},
   year={2015}
}

@ARTICLE{Marsset2019,
       author = {{Marsset}, Micha{\"e}l and {DeMeo}, Francesca and {Sonka}, Adrian and {Birlan}, Mirel and {Polishook}, David and {Burt}, Brian and {Binzel}, Richard P. and {Bus}, Shelte J. and {Thomas}, Cristina},
        title = "{Active Asteroid (6478) Gault: A Blue Q-type Surface below the Dust?}",
      journal = {\apjl},
     keywords = {Asteroids, Spectroscopy, Photometry, 72, 1558, 1234, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = sep,
       volume = {882},
       number = {1},
          eid = {L2},
        pages = {L2},
          doi = {10.3847/2041-8213/ab32ee},
archivePrefix = {arXiv},
       eprint = {1907.10077},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...882L...2M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chang2016,
       author = {{Chang}, Chan-Kao and {Lin}, Hsing-Wen and {Ip}, Wing-Huen and {Prince}, Thomas A. and {Kulkarni}, Shrinivas R. and {Levitan}, David and {Laher}, Russ and {Surace}, Jason},
        title = "{Large Super-fast Rotator Hunting Using the Intermediate Palomar Transient Factory}",
      journal = {\apjs},
     keywords = {minor planets, asteroids: general, surveys, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = dec,
       volume = {227},
       number = {2},
          eid = {20},
        pages = {20},
          doi = {10.3847/0067-0049/227/2/20},
archivePrefix = {arXiv},
       eprint = {1608.07910},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..227...20C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chang2017,
       author = {{Chang}, Chan-Kao and {Lin}, Hsing-Wen and {Ip}, Wing-Huen and {Lin}, Zhong-Yi and {Kupfer}, Thomas and {Prince}, Thomas A. and {Ye}, Quan-Zhi and {Laher}, Russ R. and {Lee}, Hee-Jae and {Moon}, Hong-Kyu},
        title = "{Confirmation of Large Super-fast Rotator (144977) 2005 EC$_{127}$}",
      journal = {\apjl},
     keywords = {minor planets, asteroids: individual: 144977 2005 EC127, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = may,
       volume = {840},
       number = {2},
          eid = {L22},
        pages = {L22},
          doi = {10.3847/2041-8213/aa6ff5},
archivePrefix = {arXiv},
       eprint = {1704.08451},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...840L..22C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chang2019,
       author = {{Chang}, Chan-Kao and {Lin}, Hsing-Wen and {Ip}, Wing-Huen and {Chen}, Wen-Ping and {Yeh}, Ting-Shuo and {Chambers}, K.~C. and {Magnier}, E.~A. and {Huber}, M.~E. and {Flewelling}, H.~A. and {Waters}, C.~Z. and {Wainscoat}, R.~J. and {Schultz}, A.~S.~B.},
        title = "{Searching for Super-fast Rotators Using the Pan-STARRS 1}",
      journal = {\apjs},
     keywords = {minor planets, asteroids: general, surveys, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = mar,
       volume = {241},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.3847/1538-4365/ab01fe},
archivePrefix = {arXiv},
       eprint = {1901.08719},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..241....6C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{Ye_2019,
	doi = {10.3847/2041-8213/ab0f3c},
	url = {https://doi.org/10.3847%2F2041-8213%2Fab0f3c},
	year = 2019,
	month = {mar},
	publisher = {American Astronomical Society},
	volume = {874},
	number = {2},
	pages = {L16},
	author = {Quanzhi Ye and Michael S. P. Kelley and Dennis Bodewits and Bryce Bolin and Lynne Jones and Zhong-Yi Lin and Eric C. Bellm and Richard Dekany and Dmitry A. Duev and Steven Groom and George Helou and Shrinivas R. Kulkarni and Thomas Kupfer and Frank J. Masci and Thomas A. Prince and Maayane T. Soumagnac},
	title = {Multiple Outbursts of Asteroid (6478) Gault},
	journal = {The Astrophysical Journal},
}

@misc{Vernazza_2016,
      title={Composition of Solar System Small Bodies}, 
      author={Pierre Vernazza and Pierre Beck},
      year={2016},
      eprint={1611.08731},
      archivePrefix={arXiv},
      primaryClass={astro-ph.EP}
}

@article{Jewitt_2019b,
	doi = {10.3847/2041-8213/ab1be8},
	url = {https://doi.org/10.3847%2F2041-8213%2Fab1be8},
	year = 2019,
	month = {may},
	publisher = {American Astronomical Society},
	volume = {876},
	number = {2},
	pages = {L19},
	author = {David Jewitt and Yoonyoung Kim and Jane Luu and Jayadev Rajagopal and Ralf Kotulla and Susan Ridgway and Wilson Liu},
	title = {Episodically Active Asteroid 6478 Gault},
	journal = {The Astrophysical Journal},
}

@article{Kleyna_2019,
	doi = {10.3847/2041-8213/ab0f40},
	url = {https://doi.org/10.3847%2F2041-8213%2Fab0f40},
	year = 2019,
	month = {apr},
	publisher = {American Astronomical Society},
	volume = {874},
	number = {2},
	pages = {L20},
	author = {Jan T. Kleyna and Olivier R. Hainaut and Karen J. Meech and Henry H. Hsieh and Alan Fitzsimmons and Marco Micheli and Jacqueline V. Keane and Larry Denneau and John Tonry and Aren Heinze and Bhuwan C. Bhatt and Devendra K. Sahu and Detlef Koschny and Ken W. Smith and Harald Ebeling and Robert Weryk and Heather Flewelling and Richard J. Wainscoat},
	title = {The Sporadic Activity of (6478) Gault: A {YORP}-driven Event?},
	journal = {The Astrophysical Journal},
}

@article{Moreno_2019,
	author = {{Moreno, F.} and {Jehin, E.} and {Licandro, J.} and {Ferrais, M.} and {Moulane, Y.} and {Pozuelos, F. J.} and {Manfroid, J.} and {Devog\`ele, M.} and {Benkhaldoun, Z.} and {Moskovitz, N.} and {Popescu, M.} and {Serra-Ricart, M.} and {Cabrera-Lavers, A.} and {Monelli, M.}},
	title = {Dust properties of double-tailed active asteroid (6478) Gault},
	DOI= "10.1051/0004-6361/201935526",
	url= "https://doi.org/10.1051/0004-6361/201935526",
	journal = {A\&A},
	year = 2019,
	volume = 624,
	pages = "L14",
}

@article{Bottke_2006,
  title={The Yarkovsky and YORP effects: Implications for asteroid dynamics},
  author={Bottke Jr, William F and Vokrouhlick{\`y}, David and Rubincam, David P and Nesvorn{\`y}, David},
  journal={Annu. Rev. Earth Planet. Sci.},
  volume={34},
  pages={157--191},
  year={2006},
  publisher={Annual Reviews}
}

@article{Hui_2019,
    author = {Hui, Man-To and Kim, Yoonyoung and Gao, Xing},
    title = "{New active asteroid (6478) Gault}",
    journal = {Monthly Notices of the Royal Astronomical Society: Letters},
    volume = {488},
    number = {1},
    pages = {L143-L148},
    year = {2019},
    month = {07},
}

@article{Chambers_2016,
  title={The Pan-STARRS1 Surveys},
  author={Chambers, KC and Magnier, EA and Metcalfe, N and Flewelling, HA and Huber, ME and Waters, CZ and Denneau, L and Draper, PW and Farrow, D and Finkbeiner, DP and others},
  journal={arXiv preprint arXiv:1612.05560},
  year={2016}
}

@article{Tonry_2012,
  title={The Pan-STARRS1 photometric system},
  author={Tonry, JL and Stubbs, Christopher W and Lykke, Keith R and Doherty, Peter and Shivvers, IS and Burgett, WS and Chambers, KC and Hodapp, KW and Kaiser, N and Kudritzki, R-P and others},
  journal={The Astrophysical Journal},
  volume={750},
  number={2},
  pages={99},
  year={2012},
  publisher={IOP Publishing}
}

@article{Muinonen_2010,
  title={A three-parameter magnitude phase function for asteroids},
  author={Muinonen, Karri and Belskaya, Irina N and Cellino, Alberto and Delb{\`o}, Marco and Levasseur-Regourd, Anny-Chantal and Penttil{\"a}, Antti and Tedesco, Edward F},
  journal={Icarus},
  volume={209},
  number={2},
  pages={542--555},
  year={2010},
  publisher={Elsevier}
}

@article{Sanchez_2019,
   title={Physical Characterization of Active Asteroid (6478) Gault},
   volume={881},
   ISSN={2041-8213},
   url={http://dx.doi.org/10.3847/2041-8213/ab31ac},
   DOI={10.3847/2041-8213/ab31ac},
   number={1},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Sanchez, Juan A. and Reddy, Vishnu and Thirouin, Audrey and Wright, Edward L. and Linder, Tyler R. and Kareta, Theodore and Sharkey, Benjamin},
   year={2019},
   month={Aug},
   pages={L6}
}

@article{Lomb_1976,
  title={Least-squares frequency analysis of unequally spaced data},
  author={Lomb, Nicholas R},
  journal={Astrophysics and space science},
  volume={39},
  number={2},
  pages={447--462},
  year={1976},
  publisher={Springer}
}

@article{Bowell_1989,
  title={Application of photometric models to asteroids.},
  author={Bowell, Edward and Hapke, Bruce and Domingue, Deborah and Lumme, Kari and Peltoniemi, Jouni and Harris, Alan W},
  journal={aste},
  pages={524--556},
  year={1989}
}
@article{Pravec_2012,
  title={Absolute magnitudes of asteroids and a revision of asteroid albedo estimates from WISE thermal observations},
  author={Pravec, Petr and Harris, Alan W and Ku{\v{s}}nir{\'a}k, Peter and Gal{\'a}d, Adri{\'a}n and Hornoch, Kamil},
  journal={Icarus},
  volume={221},
  number={1},
  pages={365--387},
  year={2012},
  publisher={Elsevier}
}

@article{Lin_2020,
    author = {Lin, Zhong-Yi and Cheng, Yu-Li and Vincent, Jean-Baptiste and Zhang, Xi-Liang and Ip, Wing Huen and Chi, Hsin-Chang},
    title = "{A study of the physical properties of an active asteroid (6478 Gault)}",
    journal = {Publications of the Astronomical Society of Japan},
    volume = {72},
    number = {5},
    year = {2020},
    month = {07},
    abstract = "{In 2019 January, the appearance of asteroid 6478 Gault immediately attracted attention because this object exhibited a long and thin tail that was quite different from the usual asteroids. This unexpected morphology placed asteroid 6478 Gault into the catalogue of active asteroids. We acquired photometric and spectroscopic observations on 37 nights from 2019 January to April using several telescopes, including LOT (1 m telescope) and SLT (40 cm telescope) at Lulin Observatory, and the 2.4 m telescope at Lijiang station of Yunnan Observatory. We did not find any reliable value for the rotational period of Gault during 2.5 hr and 5 hr observations on 2019 January 26 at Lijiang station and March 25 at Lulin Observatory, respectively. We classified 6478 Gault as a Q-type asteroid using visible spectrum and photometric measurements, including colors (B − Vavg = 0.764 ± 0.045, V − Ravg = 0.450 ± 0.023), and relative reflectance. By using Finson–Probstein analysis, the grain size for Gault’s tail 2 is larger than 20 μm.}",
    issn = {0004-6264},
    doi = {10.1093/pasj/psaa069},
    url = {https://doi.org/10.1093/pasj/psaa069},
    note = {79},
    eprint = {https://academic.oup.com/pasj/article-pdf/72/5/79/33828666/psaa069.pdf},
}

@article{Harding_2016,
   title={CHIMERA: a wide-field, multi-colour, high-speed photometer at the prime focus of the Hale telescope},
   volume={457},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stw094},
   DOI={10.1093/mnras/stw094},
   number={3},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Harding, L. K. and Hallinan, G. and Milburn, J. and Gardner, P. and Konidaris, N. and Singh, N. and Shao, M. and Sandhu, J. and Kyne, G. and Schlichting, H. E.},
   year={2016},
   month={Mar},
   pages={3036–3049}
}


@article{Farinella1998,
	Author = {{Farinella}, P. and {Vokrouhlick\'y}, D. and {Hartmann}, W.~K.},
	Journal = {\icarus},
	Month = jun,
	Pages = {378-387},
	Title = {Meteorite Delivery via Yarkovsky Orbital Drift},
	Volume = 132,
	Year = 1998}

@INPROCEEDINGS{Binzel1989,
   author = {{Binzel}, R.~P. and {Farinella}, P. and {Zappal\`a}, V. and {Cellino}, A.
	},
    title = "{Asteroid rotation rates - Distributions and statistics}",
 keywords = {Asteroids, Light Curve, Planetary Rotation, Statistical Analysis, Angular Velocity, Catastrophe Theory, Planetary Evolution, Planetary Surfaces},
booktitle = {Asteroids II},
     year = 1989,
   editor = {{Binzel}, R.~P. and {Gehrels}, T. and {Matthews}, M.~S.},
    pages = {416-441},
   adsurl = {http://adsabs.harvard.edu/abs/1989aste.conf..416B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bolin2018,
   author = {{Bolin}, B.~T. and {Weaver}, H.~A. and {Fernandez}, Y.~R. and 
	{Lisse}, C.~M. and {Huppenkothen}, D. and {Jones}, R.~L. and 
	{Juri{\'c}}, M. and {Moeyens}, J. and {Schambeau}, C.~A. and 
	{Slater}, C.~T. and {Ivezi{\'c}}, {\v Z}. and {Connolly}, A.~J.
	},
    title = "{APO Time-resolved Color Photometry of Highly Elongated Interstellar Object 1I' Oumuamua}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1711.04927},
 primaryClass = "astro-ph.EP",
 keywords = {local interstellar matter, minor planets, asteroids: individual: 1I{\amp}2017 U1 'Oumuamua},
     year = 2018,
    month = jan,
   volume = 852,
      eid = {L2},
    pages = {L2},
      doi = {10.3847/2041-8213/aaa0c9},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...852L...2B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moreno2017,
   author = {{Moreno}, F. and {Pozuelos}, F.~J. and {Novakovi{\'c}}, B. and 
	{Licandro}, J. and {Cabrera-Lavers}, A. and {Bolin}, B. and 
	{Jedicke}, R. and {Gladman}, B.~J. and {Bannister}, M.~T. and 
	{Gwyn}, S.~D.~J. and {Vere{\v s}}, P. and {Chambers}, K. and 
	{Chastel}, S. and {Denneau}, L. and {Flewelling}, H. and {Huber}, M. and 
	{Schunov{\'a}-Lilly}, E. and {Magnier}, E. and {Wainscoat}, R. and 
	{Waters}, C. and {Weryk}, R. and {Farnocchia}, D. and {Micheli}, M.
	},
    title = "{The Splitting of Double-component Active Asteroid P/2016 J1 (PANSTARRS)}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1702.03665},
 primaryClass = "astro-ph.EP",
 keywords = {methods: numerical, minor planets, asteroids: indivdual: P/2016 J1 (PANSTARRS)},
     year = 2017,
    month = mar,
   volume = 837,
      eid = {L3},
    pages = {L3},
      doi = {10.3847/2041-8213/aa6036},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...837L...3M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jewitt2017,
   author = {{Jewitt}, D. and {Agarwal}, J. and {Li}, J. and {Weaver}, H. and 
	{Mutchler}, M. and {Larson}, S.},
    title = "{Anatomy of an Asteroid Breakup: The Case of P/2013 R3}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1703.09668},
 primaryClass = "astro-ph.EP",
 keywords = {comets: general, minor planets, asteroids: general, minor planets, asteroids: individual: P{\amp}2013 R3},
     year = 2017,
    month = may,
   volume = 153,
      eid = {223},
    pages = {223},
      doi = {10.3847/1538-3881/aa6a57},
   adsurl = {http://adsabs.harvard.edu/abs/2017AJ....153..223J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bottke2005b,
   author = {{Bottke}, W.~F. and {Durda}, D.~D. and {Nesvorn{\'y}}, D. and 
	{Jedicke}, R. and {Morbidelli}, A. and {Vokrouhlick{\'y}}, D. and 
	{Levison}, H.~F.},
    title = "{Linking the collisional history of the main asteroid belt to its dynamical excitation and depletion}",
  journal = {\icarus},
     year = 2005,
    month = dec,
   volume = 179,
    pages = {63-94},
      doi = {10.1016/j.icarus.2005.05.017},
   adsurl = {http://adsabs.harvard.edu/abs/2005Icar..179...63B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Hirabayashi_2020,
   title={Spin-driven evolution of asteroids’ top-shapes at fast and slow spins seen from (101955) Bennu and (162173) Ryugu},
   volume={352},
   ISSN={0019-1035},
   url={http://dx.doi.org/10.1016/j.icarus.2020.113946},
   DOI={10.1016/j.icarus.2020.113946},
   journal={Icarus},
   publisher={Elsevier BV},
   author={Hirabayashi, Masatoshi and Nakano, Ryota and Tatsumi, Eri and Walsh, Kevin J. and Barnouin, Olivier S. and Michel, Patrick and Hartzell, Christine M. and Britt, Daniel T. and Sugita, Seiji and Watanabe, Sei-ichiro and et al.},
   year={2020},
   month={Dec},
   pages={113946}
}

@article{Taylor_2019,
   title={Arecibo radar observations of near-Earth asteroid (3200) Phaethon during the 2017 apparition},
   volume={167},
   ISSN={0032-0633},
   url={http://dx.doi.org/10.1016/j.pss.2019.01.009},
   DOI={10.1016/j.pss.2019.01.009},
   journal={Planetary and Space Science},
   publisher={Elsevier BV},
   author={Taylor, Patrick A. and Rivera-Valentín, Edgard G. and Benner, Lance A.M. and Marshall, Sean E. and Virkki, Anne K. and Venditti, Flaviane C.F. and Zambrano-Marin, Luisa F. and Bhiravarasu, Sriram S. and Aponte-Hernandez, Betzaida and Rodriguez Sanchez-Vahamonde, Carolina and et al.},
   year={2019},
   month={Mar},
   pages={1–8}
}

@article{Kim_2018,
  title={Optical observations of NEA 3200 Phaethon (1983 TB) during the 2017 apparition},
  author={Kim, M-J and Lee, H-J and Lee, S-M and Kim, D-H and Yoshida, Fumi and Bartczak, Przemyslaw and Dudzi{\'n}ski, G and Park, Jintae and Choi, Y-J and Moon, H-K and others},
  journal={Astronomy \& Astrophysics},
  volume={619},
  pages={A123},
  year={2018},
  publisher={EDP Sciences}
}

@article{Jewitt_2019,
  title={High-resolution Thermal Infrared Imaging of 3200 Phaethon},
  author={Jewitt, David and Asmus, Daniel and Yang, Bin and Li, Jing},
  journal={The Astronomical Journal},
  volume={157},
  number={5},
  pages={193},
  year={2019},
  publisher={IOP Publishing}
}

@INPROCEEDINGS{Dekany2016,
       author = {{Dekany}, Richard and {Smith}, Roger M. and {Belicki}, Justin and
         {Delacroix}, Alexandre and {Duggan}, Gina and {Feeney}, Michael and
         {Hale}, David and {Kaye}, Stephen and {Milburn}, Jennifer and
         {Murphy}, Patrick and {Porter}, Michael and {Reiley}, Daniel J. and
         {Riddle}, Reed L. and {Rodriguez}, Hector and {Bellm}, Eric C.},
        title = "{The Zwicky Transient Facility Camera}",
    booktitle = {\procspie},
         year = 2016,
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9908},
        month = aug,
          eid = {99085M},
        pages = {99085M},
          doi = {10.1117/12.2234558},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SPIE.9908E..5MD},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dekany2020,
       author = {{Dekany}, Richard and {Smith}, Roger M. and {Riddle}, Reed and {Feeney}, Michael and {Porter}, Michael and {Hale}, David and {Zolkower}, Jeffry and {Belicki}, Justin and {Kaye}, Stephen and {Henning}, John and {Walters}, Richard and {Cromer}, John and {Delacroix}, Alex and {Rodriguez}, Hector and {Reiley}, Daniel J. and {Mao}, Peter and {Hover}, David and {Murphy}, Patrick and {Burruss}, Rick and {Baker}, John and {Kowalski}, Marek and {Reif}, Klaus and {Mueller}, Phillip and {Bellm}, Eric and {Graham}, Matthew and {Kulkarni}, Shrinivas R.},
        title = "{The Zwicky Transient Facility: Observing System}",
      journal = {\pasp},
     keywords = {instrumentation: detectors, instrumentation: miscellaneous, methods: observational, surveys, techniques: photometric, time, Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Instrumentation and Detectors, Physics - Optics},
         year = 2020,
        month = mar,
       volume = {132},
       number = {1009},
          eid = {038001},
        pages = {038001},
          doi = {10.1088/1538-3873/ab4ca2},
archivePrefix = {arXiv},
       eprint = {2008.04923},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020PASP..132c8001D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kasliwal2019,
       author = {{Kasliwal}, M.~M. and {Cannella}, C. and {Bagdasaryan}, A. and
         {Hung}, T. and {Feindt}, U. and {Singer}, L.~P. and {Coughlin}, M. and
         {Fremling}, C. and {Walters}, R. and {Duev}, D. and {Itoh}, R. and
         {Quimby}, R.~M.},
        title = "{The GROWTH Marshal: A Dynamic Science Portal for Time-domain Astronomy}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Mar",
       volume = {131},
       number = {997},
        pages = {038003},
          doi = {10.1088/1538-3873/aafbc2},
archivePrefix = {arXiv},
       eprint = {1902.01934},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131c8003K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hanus2018,
   author = {{Hanu{\v s}}, J. and {Delbo}, M. and {Al{\'{\i}}-Lagoa}, V. and 
	{Bolin}, B. and {Jedicke}, R. and {{\v D}urech}, J. and {Cibulkov{\'a}}, H. and 
	{Pravec}, P. and {Ku{\v s}nir{\'a}k}, P. and {Behrend}, R. and 
	{Marchis}, F. and {Antonini}, P. and {Arnold}, L. and {Audejean}, M. and 
	{Bachschmidt}, M. and {Bernasconi}, L. and {Brunetto}, L. and 
	{Casulli}, S. and {Dymock}, R. and {Esseiva}, N. and {Esteban}, M. and 
	{Gerteis}, O. and {de Groot}, H. and {Gully}, H. and {Hamanowa}, H. and 
	{Hamanowa}, H. and {Krafft}, P. and {Lehk{\'y}}, M. and {Manzini}, F. and 
	{Michelet}, J. and {Morelle}, E. and {Oey}, J. and {Pilcher}, F. and 
	{Reignier}, F. and {Roy}, R. and {Salom}, P.~A. and {Warner}, B.~D.
	},
    title = "{Spin states of asteroids in the Eos collisional family}",
  journal = {\icarus},
archivePrefix = "arXiv",
   eprint = {1707.05507},
 primaryClass = "astro-ph.EP",
 keywords = {Asteroids, Asteroids rotation, Photometry},
     year = 2018,
    month = jan,
   volume = 299,
    pages = {84-96},
      doi = {10.1016/j.icarus.2017.07.007},
   adsurl = {http://adsabs.harvard.edu/abs/2018Icar..299...84H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Graham_2019,
	doi = {10.1088/1538-3873/ab006c},
	url = {https://doi.org/10.1088/1538-3873/ab006c},
	year = 2019,
	month = {may},
	publisher = {{IOP} Publishing},
	volume = {131},
	number = {1001},
	pages = {078001},
	author = {Matthew J. Graham and S. R. Kulkarni and Eric C. Bellm and Scott M. Adams and Cristina Barbarino and Nadejda Blagorodnova and Dennis Bodewits and Bryce Bolin and Patrick R. Brady and S. Bradley Cenko and Chan-Kao Chang and Michael W. Coughlin and Kishalay De and Gwendolyn Eadie and Tony L. Farnham and Ulrich Feindt and Anna Franckowiak and Christoffer Fremling and Suvi Gezari and Shaon Ghosh and Daniel A. Goldstein and V. Zach Golkhou and Ariel Goobar and Anna Y. Q. Ho and Daniela Huppenkothen and {\v{Z}}eljko Ivezi{\'{c}} and R. Lynne Jones and Mario Juric and David L. Kaplan and Mansi M. Kasliwal and Michael S. P. Kelley and Thomas Kupfer and Chien-De Lee and Hsing Wen Lin and Ragnhild Lunnan and Ashish A. Mahabal and Adam A. Miller and Chow-Choong Ngeow and Peter Nugent and Eran O. Ofek and Thomas A. Prince and Ludwig Rauch and Jan van Roestel and Steve Schulze and Leo P. Singer and Jesper Sollerman and Francesco Taddia and Lin Yan and Quan-Zhi Ye and Po-Chieh Yu and Tom Barlow and James Bauer and Ron Beck and Justin Belicki and Rahul Biswas and Valery Brinnel and Tim Brooke and Brian Bue and Mattia Bulla and Rick Burruss and Andrew Connolly and John Cromer and Virginia Cunningham and Richard Dekany and Alex Delacroix and Vandana Desai and Dmitry A. Duev and Michael Feeney and David Flynn and Sara Frederick and Avishay Gal-Yam and Matteo Giomi and Steven Groom and Eugean Hacopians and David Hale and George Helou and John Henning and David Hover and Lynne A. Hillenbrand and Justin Howell and Tiara Hung and David Imel and Wing-Huen Ip and Edward Jackson and Shai Kaspi and Stephen Kaye and Marek Kowalski and Emily Kramer and Michael Kuhn and Walter Landry and Russ R. Laher and Peter Mao and Frank J. Masci and Serge Monkewitz and Patrick Murphy and Jakob Nordin and Maria T. Patterson and Bryan Penprase and Michael Porter and Umaa Rebbapragada and Dan Reiley and Reed Riddle and Mickael Rigault and Hector Rodriguez and Ben Rusholme and Jakob van Santen and David L. Shupe and Roger M. Smith and Maayane T. Soumagnac and Robert Stein and Jason Surace and Paula Szkody and Scott Terek and Angela Van Sistine and Sjoert van Velzen and W. Thomas Vestrand and Richard Walters and Charlotte Ward and Chaoran Zhang and Jeffry Zolkower},
	title = {The Zwicky Transient Facility: Science Objectives},
	journal = {Publications of the Astronomical Society of the Pacific},
}

@article{Masci_2018,
	doi = {10.1088/1538-3873/aae8ac},
	url = {https://doi.org/10.1088/1538-3873/aae8ac},
	year = 2018,
	month = {dec},
	publisher = {{IOP} Publishing},
	volume = {131},
	number = {995},
	pages = {018003},
	author = {Frank J. Masci and Russ R. Laher and Ben Rusholme and David L. Shupe and Steven Groom and Jason Surace and Edward Jackson and Serge Monkewitz and Ron Beck and David Flynn and Scott Terek and Walter Landry and Eugean Hacopians and Vandana Desai and Justin Howell and Tim Brooke and David Imel and Stefanie Wachter and Quan-Zhi Ye and Hsing-Wen Lin and S. Bradley Cenko and Virginia Cunningham and Umaa Rebbapragada and Brian Bue and Adam A. Miller and Ashish Mahabal and Eric C. Bellm and Maria T. Patterson and Mario Juri{\'{c}} and V. Zach Golkhou and Eran O. Ofek and Richard Walters and Matthew Graham and Mansi M. Kasliwal and Richard G. Dekany and Thomas Kupfer and Kevin Burdge and Christopher B. Cannella and Tom Barlow and Angela Van Sistine and Matteo Giomi and Christoffer Fremling and Nadejda Blagorodnova and David Levitan and Reed Riddle and Roger M. Smith and George Helou and Thomas A. Prince and Shrinivas R. Kulkarni},
	title = {The Zwicky Transient Facility: Data Processing, Products, and Archive},
	journal = {Publications of the Astronomical Society of the Pacific},
}



@ARTICLE{Masci2019,
   author = {{Masci}, F.~J. and {Laher}, R.~R. and {Rusholme}, B. and {Shupe}, D.~L. and 
	{Groom}, S. and {Surace}, J. and {Jackson}, E. and {Monkewitz}, S. and 
	{Beck}, R. and {Flynn}, D. and {Terek}, S. and {Landry}, W. and 
	{Hacopians}, E. and {Desai}, V. and {Howell}, J. and {Brooke}, T. and 
	{Imel}, D. and {Wachter}, S. and {Ye}, Q.-Z. and {Lin}, H.-W. and 
	{Cenko}, S.~B. and {Cunningham}, V. and {Rebbapragada}, U. and 
	{Bue}, B. and {Miller}, A.~A. and {Mahabal}, A. and {Bellm}, E.~C. and 
	{Patterson}, M.~T. and {Juri{\'c}}, M. and {Golkhou}, V.~Z. and 
	{Ofek}, E.~O. and {Walters}, R. and {Graham}, M. and {Kasliwal}, M.~M. and 
	{Dekany}, R.~G. and {Kupfer}, T. and {Burdge}, K. and {Cannella}, C.~B. and 
	{Barlow}, T. and {Van Sistine}, A. and {Giomi}, M. and {Fremling}, C. and 
	{Blagorodnova}, N. and {Levitan}, D. and {Riddle}, R. and {Smith}, R.~M. and 
	{Helou}, G. and {Prince}, T.~A. and {Kulkarni}, S.~R.},
    title = "{The Zwicky Transient Facility: Data Processing, Products, and Archive}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1902.01872},
 primaryClass = "astro-ph.IM",
     year = 2019,
    month = jan,
   volume = 131,
   number = 1,
    pages = {018003},
      doi = {10.1088/1538-3873/aae8ac},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8003M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Bellm_2019,
	doi = {10.1088/1538-3873/aaecbe},
	url = {https://doi.org/10.1088/1538-3873/aaecbe},
	year = 2019,
	month = {dec},
	publisher = {{IOP} Publishing},
	volume = {131},
	number = {995},
	pages = {018002},
	author = {Eric C. Bellm and Shrinivas R. Kulkarni and Matthew J. Graham and Richard Dekany and Roger M. Smith and Reed Riddle and Frank J. Masci and George Helou and Thomas A. Prince and Scott M. Adams and C. Barbarino and Tom Barlow and James Bauer and Ron Beck and Justin Belicki and Rahul Biswas and Nadejda Blagorodnova and Dennis Bodewits and Bryce Bolin and Valery Brinnel and Tim Brooke and Brian Bue and Mattia Bulla and Rick Burruss and S. Bradley Cenko and Chan-Kao Chang and Andrew Connolly and Michael Coughlin and John Cromer and Virginia Cunningham and Kishalay De and Alex Delacroix and Vandana Desai and Dmitry A. Duev and Gwendolyn Eadie and Tony L. Farnham and Michael Feeney and Ulrich Feindt and David Flynn and Anna Franckowiak and S. Frederick and C. Fremling and Avishay Gal-Yam and Suvi Gezari and Matteo Giomi and Daniel A. Goldstein and V. Zach Golkhou and Ariel Goobar and Steven Groom and Eugean Hacopians and David Hale and John Henning and Anna Y. Q. Ho and David Hover and Justin Howell and Tiara Hung and Daniela Huppenkothen and David Imel and Wing-Huen Ip and {\v{Z}}eljko Ivezi{\'{c}} and Edward Jackson and Lynne Jones and Mario Juric and Mansi M. Kasliwal and S. Kaspi and Stephen Kaye and Michael S. P. Kelley and Marek Kowalski and Emily Kramer and Thomas Kupfer and Walter Landry and Russ R. Laher and Chien-De Lee and Hsing Wen Lin and Zhong-Yi Lin and Ragnhild Lunnan and Matteo Giomi and Ashish Mahabal and Peter Mao and Adam A. Miller and Serge Monkewitz and Patrick Murphy and Chow-Choong Ngeow and Jakob Nordin and Peter Nugent and Eran Ofek and Maria T. Patterson and Bryan Penprase and Michael Porter and Ludwig Rauch and Umaa Rebbapragada and Dan Reiley and Mickael Rigault and Hector Rodriguez and Jan van Roestel and Ben Rusholme and Jakob van Santen and S. Schulze and David L. Shupe and Leo P. Singer and Maayane T. Soumagnac and Robert Stein and Jason Surace and Jesper Sollerman and Paula Szkody and F. Taddia and Scott Terek and Angela Van Sistine and Sjoert van Velzen and W. Thomas Vestrand and Richard Walters and Charlotte Ward and Quan-Zhi Ye and Po-Chieh Yu and Lin Yan and Jeffry Zolkower},
	title = {The Zwicky Transient Facility: System Overview, Performance, and First Results},
	journal = {Publications of the Astronomical Society of the Pacific},
}

@MISC{Kelley_2019,
       author = {{Kelley}, Michael S.~P. and {Bodewits}, Dennis and {Ye}, Qaunzhi and {Laher}, Russ R. and {Masci}, Frank J. and {Monkewitz}, Serge and {Riddle}, Reed and {Rusholme}, Ben and {Shupe}, David L. and {Soumagnac}, Maayane T.},
        title = "{ZChecker: Zwicky Transient Facility moving target checker for short object lists}",
     keywords = {Software, NASA},
         year = 2019,
        month = jul,
          eid = {ascl:1907.017},
        pages = {ascl:1907.017},
archivePrefix = {ascl},
       eprint = {1907.017},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ascl.soft07017K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Jewitt_2017,
	doi = {10.3847/2041-8213/aa9b2f},
	url = {https://doi.org/10.3847/2041-8213/aa9b2f},
	year = 2017,
	month = {nov},
	publisher = {American Astronomical Society},
	volume = {850},
	number = {2},
	pages = {L36},
	author = {David Jewitt and Jane Luu and Jayadev Rajagopal and Ralf Kotulla and Susan Ridgway and Wilson Liu and Thomas Augusteijn},
	title = {Interstellar Interloper 1I/2017 U1: Observations from the {NOT} and {WIYN} Telescopes},
	journal = {The Astrophysical Journal},
}

@article{Smith_2019,
  title={(6478) Gault},
  author={Smith, KW and Denneau, L and Vincent, J-B and Weryk, R},
  journal={CBET},
  volume={4594},
  pages={1},
  year={2019}
}

@article{Chandler_2019,
  title={Six Years of Sustained Activity in (6478) Gault},
  author={Chandler, Colin Orion and Kueny, Jay and Gustafsson, Annika and Trujillo, Chadwick A and Robinson, Tyler D and Trilling, David E},
  journal={The Astrophysical Journal Letters},
  volume={877},
  number={1},
  pages={L12},
  year={2019},
  publisher={IOP Publishing}
}

@article{Ivanova_2020,
   title={Activity of (6478) Gault during 2019 January 13–March 28},
   volume={496},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/staa1630},
   DOI={10.1093/mnras/staa1630},
   number={3},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Ivanova, Oleksandra and Skorov, Yuri and Luk’yanyk, Igor and Tomko, Dušan and Husárik, Marek and Blum, Jürgen and Egorov, Oleg and Voziakova, Olga},
   year={2020},
   month={Jun},
   pages={2636–2647}
}

@article{Carbognani_Buzzoni_2020,
    author = {Carbognani, Albino and Buzzoni, Alberto},
    title = "{Spinning and colour properties of the active asteroid (6478) Gault}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {493},
    number = {1},
    pages = {70-77},
    year = {2020},
    month = {01},
    doi = {10.1093/mnras/staa208},
    url = {https://doi.org/10.1093/mnras/staa208},
    eprint = {https://academic.oup.com/mnras/article-pdf/493/1/70/32450980/staa208.pdf},
}

@article{Ferrin_2019,
    author = {Ferrín, Ignacio and Fornari, Cesar and Acosta, Agustín},
    title = "{Secular and rotational light curves of 6478 Gault}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {490},
    number = {1},
    pages = {219-230},
    year = {2019},
    month = {09},
    issn = {0035-8711},
    doi = {10.1093/mnras/stz2418},
    url = {https://doi.org/10.1093/mnras/stz2418},
    eprint = {https://academic.oup.com/mnras/article-pdf/490/1/219/30100405/stz2418.pdf},
}

@article{Warner_2009,
  title={The asteroid lightcurve database},
  author={Warner, Brian D and Harris, Alan W and Pravec, Petr},
  journal={Icarus},
  volume={202},
  number={1},
  pages={134--146},
  year={2009},
  publisher={Elsevier}
}


@ARTICLE{Bolin2021,
       author = {{Bolin}, Bryce T. and {Fernandez}, Yanga R. and {Lisse}, Carey M. and {Holt}, Timothy R. and {Lin}, Zhong-Yi and {Purdum}, Josiah N. and {Deshmukh}, Kunal P. and {Bauer}, James M. and {Bellm}, Eric C. and {Bodewits}, Dennis and {Burdge}, Kevin B. and {Carey}, Sean J. and {Copperwheat}, Chris M. and {Helou}, George and {Ho}, Anna Y.~Q. and {Horner}, Jonathan and {van Roestel}, Jan and {Bhalerao}, Varun and {Chang}, Chan-Kao and {Chen}, Christine and {Hsu}, Chen-Yen and {Ip}, Wing-Huen and {Kasliwal}, Mansi M. and {Masci}, Frank J. and {Ngeow}, Chow-Choong and {Quimby}, Robert and {Burruss}, Rick and {Coughlin}, Michael and {Dekany}, Richard and {Delacroix}, Alexandre and {Drake}, Andrew and {Duev}, Dmitry A. and {Graham}, Matthew and {Hale}, David and {Kupfer}, Thomas and {Laher}, Russ R. and {Mahabal}, Ashish and {Mr{\'o}z}, Przemyslaw J. and {Neill}, James D. and {Riddle}, Reed and {Rodriguez}, Hector and {Smith}, Roger M. and {Soumagnac}, Maayane T. and {Walters}, Richard and {Yan}, Lin and {Zolkower}, Jeffry},
        title = "{Initial Characterization of Active Transitioning Centaur, P/2019 LD2 (ATLAS), using Hubble, Spitzer, ZTF, Keck, APO and GROWTH Visible \& Infrared Imaging and Spectroscopy}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = nov,
          eid = {arXiv:2011.03782},
        pages = {arXiv:2011.03782},
archivePrefix = {arXiv},
       eprint = {2011.03782},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201103782B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bolin2020asdfasdf,
       author = {{Bolin}, Bryce T. and {Lisse}, Carey M. and {Kasliwal}, Mansi M. and
         {Quimby}, Robert and {Tan}, Hanjie and {Copperwheat}, Chris M. and
         {Lin}, Zhong-Yi and {Morbidelli}, Alessandro and {Abe}, Lyu and
         {Bendjoya}, Philippe and {Burdge}, Kevin B. and {Coughlin}, Michael and
         {Fremling}, Christoffer and {Itoh}, Ryosuke and {Koss}, Michael and
         {Masci}, Frank J. and {Maeno}, Syota and {Mamajek}, Eric E. and
         {Marocco}, Federico and {Murata}, Katsuhiro and {Rivet}, Jean-Pierre and
         {Sitko}, Michael L. and {Stern}, Daniel and {Vernet}, David and
         {Walters}, Richard and {Yan}, Lin and {Andreoni}, Igor and
         {Bhalerao}, Varun and {Bodewits}, Dennis and {De}, Kishalay and
         {Deshmukh}, Kunal P. and {Bellm}, Eric C. and {Blagorodnova}, Nadejda and
         {Buzasi}, Derek and {Cenko}, S. Bradley and {Chang}, Chan-Kao and
         {Chojnowski}, Drew and {Dekany}, Richard and {Duev}, Dmitry A. and
         {Graham}, Matthew and {Juri{\'c}}, Mario and {Kulkarni}, Shrinivas R. and
         {Kupfer}, Thomas and {Mahabal}, Ashish and {Neill}, James D. and
         {Ngeow}, Chow-Choong and {Penprase}, Bryan and {Riddle}, Reed and
         {Rodriguez}, Hector and {Smith}, Roger M. and {Rosnet}, Philippe and
         {Sollerman}, Jesper and {Soumagnac}, Maayane T.},
        title = "{Characterization of the Nucleus, Morphology, and Activity of Interstellar Comet 2I/Borisov by Optical and Near-infrared GROWTH, Apache Point, IRTF, ZTF, and Keck Observations}",
      journal = {\aj},
     keywords = {UAT:280, UAT:1065, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = jul,
       volume = {160},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.3847/1538-3881/ab9305},
archivePrefix = {arXiv},
       eprint = {1910.14004},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160...26B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Masiero2009,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009Icar..204..145M},
	Archiveprefix = {arXiv},
	Author = {{Masiero}, J. and {Jedicke}, R. and {{\v D}urech}, J. and {Gwyn}, S. and {Denneau}, L. and {Larsen}, J.},
	Doi = {10.1016/j.icarus.2009.06.012},
	Eprint = {0906.3339},
	Journal = {\icarus},
	Month = nov,
	Pages = {145-171},
	Primaryclass = {astro-ph.EP},
	Title = {{The Thousand Asteroid Light Curve Survey}},
	Volume = 204,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.icarus.2009.06.012}}

@ARTICLE{Jedicke2016,
   author = {{Jedicke}, R. and {Bolin}, B. and {Granvik}, M. and {Beshore}, E.
	},
    title = "{A fast method for quantifying observational selection effects in asteroid surveys}",
  journal = {\icarus},
 keywords = {Near-Earth Objects, Asteroids, dynamics, Data reduction techniques, Asteroids},
     year = 2016,
    month = mar,
   volume = 266,
    pages = {173-188},
      doi = {10.1016/j.icarus.2015.10.021},
   adsurl = {http://adsabs.harvard.edu/abs/2016Icar..266..173J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bolin2014,
   author = {{Bolin}, B. and {Jedicke}, R. and {Granvik}, M. and {Brown}, P. and 
	{Howell}, E. and {Nolan}, M.~C. and {Jenniskens}, P. and {Chyba}, M. and 
	{Patterson}, G. and {Wainscoat}, R.},
    title = "{Detecting Earth's temporarily-captured natural satellites-Minimoons}",
  journal = {\icarus},
archivePrefix = "arXiv",
   eprint = {1406.3534},
 primaryClass = "astro-ph.EP",
     year = 2014,
    month = oct,
   volume = 241,
    pages = {280-297},
      doi = {10.1016/j.icarus.2014.05.026},
   adsurl = {http://adsabs.harvard.edu/abs/2014Icar..241..280B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sanchez2014,
   author = {{S\'{a}nchez}, P. and {Scheeres}, D.~J.},
    title = "{The strength of regolith and rubble pile asteroids}",
  journal = {Meteoritics and Planetary Science},
archivePrefix = "arXiv",
   eprint = {1306.1622},
 primaryClass = "astro-ph.EP",
     year = 2014,
    month = may,
   volume = 49,
    pages = {788-811},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Pravec2008,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008Icar..197..497P},
	Author = {{Pravec}, P. and {Harris}, A.~W. and {Vokrouhlick{\'y}}, D. and {Warner}, B.~D. and {Ku{\v s}nir{\'a}k}, P. and {Hornoch}, K. and {Pray}, D.~P. and {Higgins}, D. and {Oey}, J. and {Gal{\'a}d}, A. and {Gajdo{\v s}}, {\v S}. and {Korno{\v s}}, L. and {Vil{\'a}gi}, J. and {Hus{\'a}rik}, M. and {Krugly}, Y.~N. and {Shevchenko}, V. and {Chiorny}, V. and {Gaftonyuk}, N. and {Cooney}, W.~R. and {Gross}, J. and {Terrell}, D. and {Stephens}, R.~D. and {Dyvig}, R. and {Reddy}, V. and {Ries}, J.~G. and {Colas}, F. and {Lecacheux}, J. and {Durkee}, R. and {Masi}, G. and {Koff}, R.~A. and {Goncalves}, R.},
	Date-Added = {2013-10-09 15:43:56 -1000},
	Date-Modified = {2013-10-09 15:43:56 -1000},
	Doi = {10.1016/j.icarus.2008.05.012},
	Journal = {\icarus},
	Month = oct,
	Pages = {497-504},
	Title = {{Spin rate distribution of small asteroids}},
	Volume = 197,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.icarus.2008.05.012}}


@article{Bolin2020CD3,
	year = 2020,
	month = {sep},
	volume = {900},
	number = {2},
	pages = {L45},
	author = {Bryce T. Bolin and Christoffer Fremling and Timothy R. Holt and Matthew J. Hankins and Tom{\'{a}}s Ahumada and Shreya Anand and Varun Bhalerao and Kevin B. Burdge and Chris M. Copperwheat and Michael Coughlin and Kunal P. Deshmukh and Kishalay De and Mansi M. Kasliwal and Alessandro Morbidelli and Josiah N. Purdum and Robert Quimby and Dennis Bodewits and Chan-Kao Chang and Wing-Huen Ip and Chen-Yen Hsu and Russ R. Laher and Zhong-Yi Lin and Carey M. Lisse and Frank J. Masci and Chow-Choong Ngeow and Hanjie Tan and Chengxing Zhai and Rick Burruss and Richard Dekany and Alexandre Delacroix and Dmitry A. Duev and Matthew Graham and David Hale and Shrinivas R. Kulkarni and Thomas Kupfer and Ashish Mahabal and Przemyslaw J. Mr{\'{o}}z and James D. Neill and Reed Riddle and Hector Rodriguez and Roger M. Smith and Maayane T. Soumagnac and Richard Walters and Lin Yan and Jeffry Zolkower},
	title = {Characterization of Temporarily Captured Minimoon 2020 {CD}3 by Keck Time-resolved Spectrophotometry},
      journal = {\apjl},
}

@ARTICLE{Vokrouhlicky2017a,
   author = {{Vokrouhlick{\'y}}, D. and {Pravec}, P. and {Durech}, J. and 
	{Bolin}, B. and {Jedicke}, R. and {Ku{\v s}nir{\'a}k}, P. and 
	{Gal{\'a}d}, A. and {Hornoch}, K. and {Kryszczy{\'n}ska}, A. and 
	{Colas}, F. and {Moskovitz}, N. and {Thirouin}, A. and {Nesvorn{\'y}}, D.
	},
    title = "{The young Datura asteroid family. Spins, shapes, and population estimate}",
  journal = {\aap},
 keywords = {celestial mechanics, minor planets, asteroids: general},
     year = 2017,
    month = feb,
   volume = 598,
      eid = {A91},
    pages = {A91},
      doi = {10.1051/0004-6361/201629670},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...598A..91V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Delbo2014,
   author = {{Delbo}, M. and {Libourel}, G. and {Wilkerson}, J. and {Murdoch}, N. and 
	{Michel}, P. and {Ramesh}, K.~T. and {Ganino}, C. and {Verati}, C. and 
	{Marchi}, S.},
    title = "{Thermal fatigue as the origin of regolith on small asteroids}",
  journal = {\nat},
     year = 2014,
    month = apr,
   volume = 508,
    pages = {233-236},
      doi = {10.1038/nature13153},
   adsurl = {http://adsabs.harvard.edu/abs/2014Natur.508..233D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Hanus2016a,
   author = {{Hanu\v{s}}, J. and {Delbo}, M. and {Vokrouhlick{\'y}}, D. and 
	{Pravec}, P. and {Emery}, J.~P. and {Al{\'{\i}}-Lagoa}, V. and 
	{Bolin}, B. and {Devog{\`e}le}, M. and {Dyvig}, R. and {Gal{\'a}d}, A. and 
	{Jedicke}, R. and {Korno{\v s}}, L. and {Ku{\v s}nir{\'a}k}, P. and 
	{Licandro}, J. and {Reddy}, V. and {Rivet}, J.-P. and {Vil{\'a}gi}, J. and 
	{Warner}, B.~D.},
    title = "{Near-Earth asteroid (3200) Phaethon: Characterization of its orbit, spin state, and thermophysical parameters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1605.05205},
 primaryClass = "astro-ph.EP",
 keywords = {minor planets, asteroids: individual: (3200) Phaethon, techniques: photometric, methods: observational, methods: numerical},
     year = 2016,
    month = jul,
   volume = 592,
      eid = {A34},
    pages = {A34},
      doi = {10.1051/0004-6361/201628666},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...592A..34H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Zappala_1990,
  title={An analysis of the amplitude-phase relationship among asteroids},
  author={Zappala, V and Cellino, A and Barucci, AM and Fulchignoni, M and Lupishko, DF},
  journal={Astronomy and Astrophysics},
  volume={231},
  pages={548--560},
  year={1990}
}

@article{Gwyn_2012,
   title={THE CANADA-FRANCE-HAWAII TELESCOPE LEGACY SURVEY: STACKED IMAGES AND CATALOGS},
   volume={143},
   ISSN={1538-3881},
   url={http://dx.doi.org/10.1088/0004-6256/143/2/38},
   DOI={10.1088/0004-6256/143/2/38},
   number={2},
   journal={The Astronomical Journal},
   publisher={American Astronomical Society},
   author={Gwyn, Stephen D. J.},
   year={2012},
   month={Jan},
   pages={38}
}

@article{Milani_2017,
  title={On the ages of resonant, eroded and fossil asteroid families},
  author={Milani, Andrea and Kne{\v{z}}evi{\'c}, Zoran and Spoto, Federica and Cellino, Alberto and Novakovi{\'c}, Bojan and Tsirvoulis, Georgios},
  journal={Icarus},
  volume={288},
  pages={240--264},
  year={2017},
  publisher={Elsevier}
}

@article{Harris_2014,
title = "On the maximum amplitude of harmonics of an asteroid lightcurve",
journal = "Icarus",
volume = "235",
pages = "55 - 59",
year = "2014",
issn = "0019-1035",
doi = "https://doi.org/10.1016/j.icarus.2014.03.004",
url = "http://www.sciencedirect.com/science/article/pii/S0019103514001213",
author = "A.W. Harris and P. Pravec and A. Galád and B.A. Skiff and B.D. Warner and J. Világi and Š. Gajdoš and A. Carbognani and K. Hornoch and P. Kušnirák and W.R. Cooney and J. Gross and D. Terrell and D. Higgins and E. Bowell and B.W. Koehn",
keywords = "Asteroids, Asteroids, rotation, Photometry",
}

@article{astropy:2013,
Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
Adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558A..33A},
Archiveprefix = {arXiv},
Author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and {Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and {Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and {Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and {Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and {Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and {Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and {Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and {Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and {Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and {Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and {Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and {Servillat}, M. and {Streicher}, O.},
Doi = {10.1051/0004-6361/201322068},
Eid = {A33},
Eprint = {1307.6212},
Journal = {\aap},
Keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
Month = oct,
Pages = {A33},
Primaryclass = {astro-ph.IM},
Title = {{Astropy: A community Python package for astronomy}},
Volume = 558,
Year = 2013,
Bdsk-Url-1 = {https://dx.doi.org/10.1051/0004-6361/201322068}}

@ARTICLE{astropy_2018,
       author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and
         {Sip{H{o}}cz}, B.~M. and {G{"u}nther}, H.~M. and {Lim}, P.~L. and
         {Crawford}, S.~M. and {Conseil}, S. and {Shupe}, D.~L. and
         {Craig}, M.~W. and {Dencheva}, N. and {Ginsburg}, A. and {Vand
        erPlas}, J.~T. and {Bradley}, L.~D. and {P{'e}rez-Su{'a}rez}, D. and
         {de Val-Borro}, M. and {Aldcroft}, T.~L. and {Cruz}, K.~L. and
         {Robitaille}, T.~P. and {Tollerud}, E.~J. and {Ardelean}, C. and
         {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and {Bakanov}, A.~V. and
         {Bamford}, S.~P. and {Barentsen}, G. and {Barmby}, P. and
         {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and {Boquien}, M. and
         {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and
         {Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and
         {Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{'i}guez}, J.~L. and
         {Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and
         {Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and
         {Depagne}, {'E}. and {Dietrich}, J.~P. and {Donath}, A. and
         {Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and
         {Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and
         {Garrison}, L.~H. and {Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and
         {Gommers}, R. and {Greco}, J.~P. and {Greenfield}, P. and
         {Groener}, A.~M. and {Grollier}, F. and {Hagen}, A. and {Hirst}, P. and
         {Homeier}, D. and {Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and
         {Hunkeler}, J.~S. and {Ivezi{'c}}, {{Z}}. and {Jain}, A. and
         {Jenness}, T. and {Kanarek}, G. and {Kendrew}, S. and {Kern}, N.~S. and
         {Kerzendorf}, W.~E. and {Khvalko}, A. and {King}, J. and {Kirkby}, D. and
         {Kulkarni}, A.~M. and {Kumar}, A. and {Lee}, A. and {Lenz}, D. and
         {Littlefair}, S.~P. and {Ma}, Z. and {Macleod}, D.~M. and
         {Mastropietro}, M. and {McCully}, C. and {Montagnac}, S. and
         {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and {Muna}, D. and
         {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and
         {Ninan}, J.~P. and {N{"o}the}, M. and {Ogaz}, S. and {Oh}, S. and
         {Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and
         {Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and
         {Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and
         {Sakurikar}, P. and {Seifert}, M. and {Sherbert}, L.~E. and
         {Sherwood-Taylor}, H. and {Shih}, A.~Y. and {Sick}, J. and
         {Silbiger}, M.~T. and {Singanamalla}, S. and {Singer}, L.~P. and
         {Sladen}, P.~H. and {Sooley}, K.~A. and {Sornarajah}, S. and
         {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and
         {Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{'o}n}, V. and
         {van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and
         {Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and
         {Zabalza}, V. and {Astropy Contributors}},
        title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
      journal = {aj},
     keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = sep,
       volume = {156},
       number = {3},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-3881/aabc4f},
archivePrefix = {arXiv},
       eprint = {1801.02634},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Laher_2012,
	doi = {10.1086/666883},
	url = {https://doi.org/10.1086/666883},
	year = 2012,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {124},
	number = {917},
	pages = {737--763},
	author = {Russ R. Laher and Varoujan Gorjian and Luisa M. Rebull and Frank J. Masci and John W. Fowler and George Helou and Shrinivas R. Kulkarni and Nicholas M. Law},
	title = {Aperture Photometry Tool},
	journal = {Publications of the Astronomical Society of the Pacific},
}

@inproceedings{Huehnerhoff_2016,
author = {Huehnerhoff, Joseph and Ketzeback, W. and Bradley, Alaina and Dembicky, Jack and Doughty, Caitlin and Hawley, Suzanne and Johnson, Courtney and Klaene, Mark and Leon, Ed and McMillan, Russet and Owen, Russell and Sayres, Conor and Sheen, Tyler and Shugart, Alysha},
year = {2016},
month = {08},
pages = {99085H},
title = {Astrophysical Research Consortium Telescope Imaging Camera (ARCTIC) facility optical imager for the Apache Point Observatory 3.5m telescope},
doi = {10.1117/12.2234214}
}

@inproceedings{Boulade_2003,
author = {Olivier Boulade and Xavier Charlot and P. Abbon and Stephan Aune and Pierre Borgeaud and Pierre-Henri Carton and M. Carty and J. Da Costa and H. Deschamps and D. Desforge and Dominique Eppelle and Pascal Gallais and L. Gosset and Remy Granelli and Michel Gros and Jean de Kat and Denis Loiseau and J. -L. Ritou and Jean Yves Rousse and Pierre Starzynski and Nicolas Vignal and Laurent G. Vigroux},
title = {{Megacam: the new Canada-France-Hawaii Telescope wide-field imaging camera}},
volume = {4841},
booktitle = {Instrument Design and Performance for Optical/Infrared Ground-based Telescopes},
editor = {Masanori Iye and Alan F. M. Moorwood},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {72 -- 81},
keywords = {Wide-field imaging camera, CCD mosaic, CCD characterization, CCD controller, cryocooler, filter juk},
year = {2003},
doi = {10.1117/12.459890},
URL = {https://doi.org/10.1117/12.459890}
}

@MISC{vizier,
author = { Ochsenbein F. et. al}
title = "{ The VizieR database of astronomical catalogues }"
doi = {10.26093/cds/vizier}, 
}

@MISC{2019ascl.soft07032M,
   author = {{McCully}, C. and {Tewes}, M.},
    title = "{Astro-SCRAPPY: Speedy Cosmic Ray Annihilation Package in Python}",
 keywords = {Software },
howpublished = {Astrophysics Source Code Library},
     year = 2019,
    month = jul,
archivePrefix = "ascl",
   eprint = {1907.032},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2019ascl.soft07032M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2018AAS...23143601F,
   author = {{Flewelling}, H.},
    title = "{Pan-STARRS Data Release 2}",
booktitle = {American Astronomical Society Meeting Abstracts \#231},
     year = 2018,
   series = {American Astronomical Society Meeting Abstracts},
   volume = 231,
    month = jan,
      eid = {436.01},
    pages = {436.01},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2018AAS...23143601F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{bertin11,
       author = {{Bertin}, E.},
        title = "{Automated Morphometry with SExtractor and PSFEx}",
    booktitle = {Astronomical Data Analysis Software and Systems XX},
         year = "2011",
       editor = {{Evans}, I.~N. and {Accomazzi}, A. and {Mink}, D.~J. and {Rots}, A.~H.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {442},
        month = "Jul",
        pages = {435},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ASPC..442..435B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Snodgrass_2010,
  title={A collision in 2009 as the origin of the debris trail of asteroid P/2010 A2},
  author={Snodgrass, Colin and Tubiana, Cecilia and Vincent, Jean-Baptiste and Sierks, Holger and Hviid, Stubbe and Moissl, Richard and Boehnhardt, Hermann and Barbieri, Cesare and Koschny, Detlef and Lamy, Philippe and others},
  journal={Nature},
  volume={467},
  number={7317},
  pages={814--816},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{Jewitt_2013,
	doi = {10.1088/2041-8205/778/1/l21},
	url = {https://doi.org/10.1088/2041-8205/778/1/l21},
	year = 2013,
	month = {nov},
	publisher = {American Astronomical Society},
	volume = {778},
	number = {1},
	pages = {L21},
	author = {David Jewitt and Jessica Agarwal and Harold Weaver and Max Mutchler and Stephen Larson},
	title = {{THE} {EXTRAORDINARY} {MULTI}-{TAILED} {MAIN}-{BELT} {COMET} P/2013 P5},
	journal = {The Astrophysical Journal},
}

@article{Lang_2010,
	doi = {10.1088/0004-6256/139/5/1782},
	url = {https://doi.org/10.1088/0004-6256/139/5/1782},
	year = 2010,
	month = {mar},
	publisher = {American Astronomical Society},
	volume = {139},
	number = {5},
	pages = {1782--1800},
	author = {Dustin Lang and David W. Hogg and Keir Mierle and Michael Blanton and Sam Roweis},
	title = {{ASTROMETRY}.{NET}: {BLIND} {ASTROMETRIC} {CALIBRATION} {OF} {ARBITRARY} {ASTRONOMICAL} {IMAGES}},
	journal = {The Astronomical Journal},
}

@article{CARRY_2012,
title = "Density of asteroids",
journal = "Planetary and Space Science",
volume = "73",
number = "1",
pages = "98 - 118",
year = "2012",
note = "Solar System science before and after Gaia",
issn = "0032-0633",
doi = "https://doi.org/10.1016/j.pss.2012.03.009",
url = "http://www.sciencedirect.com/science/article/pii/S0032063312000773",
author = "B. Carry",
keywords = "Minor planets, Mass, Volume, Density, Porosity",
}

@BOOK{Press_1986,
       author = {{Press}, William H. and {Flannery}, Brian P. and {Teukolsky}, Saul A.},
        title = "{Numerical recipes. The art of scientific computing}",
         year = 1986,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986nras.book.....P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
